Training-Time Attacks against k-Nearest Neighbors

Nearest neighbor-based methods are commonly used for classification tasks and as subroutines of other data-analysis methods. An attacker with the capability of inserting their own data points into the training set can manipulate the inferred nearest neighbor structure. We distill this goal to the task of performing a training-set data insertion attack against $k$-Nearest Neighbor classification ($k$NN). We prove that computing an optimal training-time (a.k.a. poisoning) attack against $k$NN classification is NP-Hard, even when $k = 1$ and the attacker can insert only a single data point. We provide an anytime algorithm to perform such an attack, and a greedy algorithm for general $k$ and attacker budget. We provide theoretical bounds and empirically demonstrate the effectiveness and practicality of our methods on synthetic and real-world datasets. Empirically, we find that $k$NN is vulnerable in practice and that dimensionality reduction is an effective defense. We conclude with a discussion of open problems illuminated by our analysis.

==> SWEEP_pseudocode.tex <==
\begin{algorithm}

  \DontPrintSemicolon
  \caption{
\sweep
    \todo{Clean up dramatically}
  }
  \label{alg:sweep}
  \SetKwFunction{FSweep}{SweepHyperspheres}
  \SetKwFunction{FSweeponeD}{Sweep-1D}
  \SetKwProg{Fn}{Function}{:}{}
  
  \KwInput{\\
    \(\trset = \{(x^{\text{tr}}, y^{\text{tr}})\}_i\): Training set
    \(\evalpool = \{(x^{\text{ev}}, y^{\text{ev}})\}_i\): Evaluation pool
    \(y\): Class of attack point to add
  }
  \KwOutput{\\
    \(\mathbf{p}\): ...}

  \(\mathbf{H}, \mathbf{L} \gets \texttt{ConstructHyperspheres}(\trset, \evalpool, y)\)\\
  Return \FSweep(\(\mathbf H\))\\
  \Fn{\FSweep}{
   \KwInput{\\%\(\mathbf H\)\\
     ~~~~ \(\mathbf H\), an ordered set of \(d\)-dimensional hyperspheres\\
     ~~~~ with centers \(\{\mathbf c_1, \ldots, \mathbf c_n\}\) and\\
     ~~~~ radii \(\{r_1, \ldots, r_n\}\).
   }
   \KwOutput {\\%\(\mathbf p\) \\
     ~~~~    \(\mathbf p\), a \(d\)-dimensional point.\\
   }
   \If {\(d = 1\)}
       { \Return \FSweeponeD (\(\mathbf H\))}
       \(\mathbf{I} \gets \{x^* ~|~ \exists h_1, h_2 \in \mathcal H \wedge x^* = \min_{x \in h_1 \cap h_2} x_0\}\)\\
       ~~~~~~\(\cup \{x^* ~|~ \exists h_1, h_2 \in \mathcal H \wedge x^* = \max_{x \in h_1 \cap h_2} x_0\}\)\\
   Sort \(\mathbf{I}\) by ascending first coordinate. \\
   \(\mathcal{M} \gets \{(I_2 - I_1)_0, (I_3 - I_2)_0, \ldots, (I_{|\mathbf I|} - I_{|\mathbf I|-1})_0\}\)\\
   \(\mathbf p = \pmb c_1\)\\
   \For{\(m  \in \mathcal{M}\)}
       {
         \(\mathbf H' \gets \mathbf H\) restricted to the hyperplane \(x_0 = m\).\\% \todo{Define restriction notation}\\
         (Note that \(\mathbf H'\) is a set of \(n\) hyperspheres in \((d-1)\) dimensions.)\\
         \(\mathbf p' \gets [m,  \FSweep(\mathbf H')]^\top\)\\
         \If{\(\mathbf p'\) is better than \(\mathbf p\)}
            {
              \(\mathbf p \gets \mathbf p'\)
            }
            
       }
       \Return \(\mathbf p\) 
 }
  \Fn{\FSweeponeD}{
    \todo{Formalize this bit}
   Solve matching parenthesis problem with standard method (just count).
 }

\end{algorithm}




==> app_pseudocode.tex <==
\input{full_atk_pseudocode}

